SSD Set System, Graph Decomposition and Hamiltonian Cycle

In this paper, we first study what we call Superset-Subset-Disjoint (SSD) set system. Based on properties of SSD set system, we derive the following (I) to (IV): (I) For a nonnegative integer $k$ and a graph $G=(V,E)$ with $|V|\ge2$, let $X_1,X_2,\dots,X_q\subsetneq V$ denote all maximal proper subsets of $V$ that induce $k$-edge-connected subgraphs. Then at least one of (a) and (b) holds: (a) $\{X_1,X_2,\dots,X_q\}$ is a partition of $V$; and (b) $V\setminus X_1, V\setminus X_2,\dots,V\setminus X_q$ are pairwise disjoint. (II) For $k=1$ and a strongly-connected digraph $G$, whether $V$ is in (a) and/or (b) can be decided in $O(n+m)$ time and we can generate all such $X_1,X_2,\dots,X_q$ in $O(n+m+|X_1|+|X_2|+\dots+|X_q|)$ time, where $n=|V|$ and $m=|E|$. (III) For a digraph $G$, we can enumerate in linear delay all vertex subsets of $V$ that induce strongly-connected subgraphs. (IV) A digraph is Hamiltonian if there is a spanning subgraph that is strongly-connected and in the case (a).

==> fig/MPSS_not_linear.tex <==
% \begin{minipage}[c]{0.5\hsize}
    \begin{tikzpicture}[entity-vertex/.style={draw, circle,minimum width=0.25cm ,inner sep=-1mm, thick}]
        % % \node[{draw, circle,minimum width=0.25cm, ,inner sep=-1mm, thick}]
        \node[entity-vertex] (v1) at ($(-36:1)+(-1.75,0)$) {};
        \node[entity-vertex] (v2) at ($(-36-72:1)+(-1.75,0)$) {};
        \node[entity-vertex,draw=white] (v3) at ($(180:1)+(-1.75,0)$) {$\vdots$};
        \node[entity-vertex] (v4) at ($(36+72:1)+(-1.75,0)$) {};
        \node[entity-vertex] (v5) at ($(36:1)+(-1.75,0)$) {};
        \draw[thick,-{Stealth}] (v1)--(v2);
        \draw[thick,-{Stealth}] (v2)--(v3);
        \draw[thick,-{Stealth}] (v3)--(v4);
        \draw[thick,-{Stealth}] (v4)--(v5);
        \draw[thick,-{Stealth}] (v5)--(v1);


        \node[entity-vertex] (u1) at ($(180-36:1)+(1.75,0)$) {};
        \node[entity-vertex] (u2) at ($(180-36-72:1)+(1.75,0)$) {};
        \node[entity-vertex,draw=white] (u3) at ($(0:1)+(1.75,0)$) {$\vdots$};
        \node[entity-vertex] (u4) at ($(180+36+72:1)+(1.75,0)$) {};
        \node[entity-vertex] (u5) at ($(180+36:1)+(1.75,0)$) {};
        \draw[thick,-{Stealth}] (u1)--(u2);
        \draw[thick,-{Stealth}] (u2)--(u3);
        \draw[thick,-{Stealth}] (u3)--(u4);
        \draw[thick,-{Stealth}] (u4)--(u5);
        \draw[thick,-{Stealth}] (u5)--(u1);

        \draw[thick,-{Stealth}] (v5)--(u1);
        \draw[thick,-{Stealth}] (u5)--(v1);

        \draw [black,very thick,dotted] (-1.75,0)circle[radius=1.25];
        \draw [black,very thick,dotted] (+1.75,0)circle[radius=1.25];
        % \draw[black,rounded corners=20,very thick]($ (u1) + (0.5,-1) $)--($ (u2) + (0.5,0.5) $)--($ (u3) + (-1,0.25) $)--cycle;
        % \draw[black,rounded corners=20,very thick]($ (u1) + (0.5,-1) $)--($ (u2) + (0.5,0.5) $)--($ (u3) + (-1,0.25) $)--cycle;
        % \draw ($ (u1) + (0.95,-1) $) node{$ Y \in \MRS_{\MC_{\mstr}}(C) $};
        % \draw ($ (v5)+(0.5, 0) $) node[red,right]{$ X = C \setminus Y $};
        % \draw[purple,rounded corners=0,very thick] (2.6, 1.75)--(-3.5, 1.75)--(-3.5, -2.25)--(2.6, -2.25)--cycle;
        \draw(-1.75, 1.5)node[black]{$ C_1 $};
        \draw(+1.75, 1.5)node[black]{$ C_2 $};
    \end{tikzpicture}
    \\ $G = (V, E)$
% \end{minipage}
% \begin{minipage}[c]{0.45\hsize}
%    Let $C_1$ and $C_2$ be directed cycles with $n / 2$ vertices. \\
%    $\MPSS(V) = \{C_1, C_2\}$. \\
%    $\sum_{} {|X|} = n$. \\
%    $\Omega(n^2 + n\sum_{} {|X|} - \sum_{} {|X|^2}) = \Omega(2n^2 - n^2/4) = \Omega(n^2) = \Omega((\sum_{} {|X|})^2)$.
   
% \end{minipage}
